Scalable Surrogate Verification of Image-based Neural Network Control Systems using Composition and Unrolling

Verifying safety of neural network control systems that use images as input is a difficult problem because, from a given system state, there is no known way to mathematically model what images are possible in the real-world. We build on recent work that considers a surrogate verification approach, training a conditional generative adversarial network (cGAN) as an image generator in place of the real world. This enables set-based formal analysis of the closed-loop system, providing analysis beyond simulation and testing. While existing work is effective on small examples, excessive overapproximation both within a single control period and across multiple control periods limits its scalability. We propose approaches to overcome these two sources of error. First, we overcome one-step error by composing the system's dynamics along with the cGAN and neural network controller, without losing the dependencies between input states and the control outputs as in the monotonic analysis of the system dynamics. Second, we reduce multi-step error by repeating the single-step composition, essentially unrolling multiple steps of the control loop into a large neural network. We then leverage existing network verification tools to compute accurate reachable sets for multiple steps, avoiding the accumulation of abstraction error at each step. We demonstrate the effectiveness of our approach in terms of both accuracy and scalability using two case studies: an autonomous aircraft taxiing system and an advanced emergency braking system. On the aircraft taxiing system, the converged reachable set is 175% larger using the prior baseline method compared with our proposed approach. On the emergency braking system, with 24x the number of image output variables from the cGAN, the baseline method fails to prove any states are safe, whereas our improvements enable set-based safety analysis.

==> checklist.tex <==
\paragraph{This paper:}
\begin{itemize}
	\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) {\bf yes}
	\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no) {\bf yes}
	\item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper (yes/no) {\bf yes}
\end{itemize}

\paragraph{Does this paper make theoretical contributions? (yes/no)} {\bf yes}

If yes, please complete the list below.
\begin{itemize}
	\item All assumptions and restrictions are stated clearly and formally. (yes/partial/no) {\bf yes}
	\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no) {\bf yes}
	\item Proofs of all novel claims are included. (yes/partial/no) {\bf yes}
	\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no) {\bf yes}
	\item Appropriate citations to theoretical tools used are given. (yes/partial/no) {\bf yes}
	\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA) {\bf yes}
	\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA) {\bf yes}
\end{itemize}

\paragraph{Does this paper rely on one or more datasets? (yes/no)} {\bf no}

If yes, please complete the list below.
\begin{itemize}
	\item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) {}
	\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) {}
	\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) {}
	\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) {}
	\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) {}
	\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) {}
\end{itemize}

\paragraph{Does this paper include computational experiments? (yes/no)} {\bf yes}

If yes, please complete the list below.
\begin{itemize}
	\item Any code required for pre-processing data is included in the appendix. (yes/partial/no) {\bf yes}
	\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) {\bf yes}
	\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) {\bf yes}
	\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. (yes/partial/no) {\bf yes}
	\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) {\bf yes}
	\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) {\bf partial}
	\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) {\bf yes}
	\item This paper states the number of algorithm runs used to compute each reported result. (yes/no) {\bf yes}
	\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) {\bf yes}
	\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) {\bf yes}
	\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) {\bf yes}
	\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) {\bf yes}
\end{itemize}

==> discussion.tex <==
\section{Limitations and Discussions}
\label{sec:limitations}
%We adopt the framework in~\cite{katz2022verification} to use a cGAN to approximate
%the actual behavior of the perception system.
The usefulness of the surrogate verification is inherently tied to the 
quality, diversity, and fidelity 
of the images generated by cGANs. 
%% quality and diversity
Despite extensive efforts to improve the visual quality and diversity of cGAN-generated images~\cite{hou2022conditional,kang2021rebooting},
these images inevitably fall short in representing the entire actual observation space.
Moreover, the intricate network architecture and numerous latent variables employed in modern cGANs challenges neural network verification tools, 
allowing only a subset of latent variables to be verifiable. 
Consequently, the verification becomes unnecessarily incomplete, potentially leading to false negatives.
%One strategy to alleviate this challenge is the conformant synthesis technique~\cite{kochdumper2022conformant}, which introduces minimal additional errors in state variables to encompass control predictions for all instances within the training dataset. While not exhaustive for the entire observation space, this technique provides formal guarantees for data from the training set.
%% fidelity
Existing strategies for enhancing diversity of the cGANs are primarily designed for categorical conditions and do not extend to the cGANs used in verifying image-based NNCS, where continuous system states serve as the condition labels.
Although continuous conditional GANs (CcGANs) \cite{ding2020ccgan} have recently been introduced to adapt cGANs to continuous condition scenarios, it may compromise label consistency to improve visual diversity.
Even without such trade-offs, our experiments indicate that cGANs can still produce images that slightly deviate from precise conditions. For example, a cGAN might generate images corresponding to ``a car positioned 4.8 meters ahead" instead of the exact condition of ``5 meters ahead."
Additionally, the process of generating images using cGANs does not consider the environmental context dependencies between consecutive image frames. If generated images from cGANs are concatenated into a sequence, each frame stands alone, and they cannot form a cohesive video. Both label inconsistency within a single frame and context inconsistency across multiple frames result in a loss of fidelity, potentially leading to false positives in verification.
%Designing a specialized cGAN that accurately captures the system state information and maintains temporal dependencies could be advantageous for surrogate verification and testing of image-based control systems.
%% 





 



